RobustNeRF: Ignoring Distractors with Robust Losses

Neural radiance fields (NeRF) excel at synthesizing new views given multi-view, calibrated images of a static scene. When scenes include distractors, which are not persistent during image capture (moving objects, lighting variations, shadows), artifacts appear as view-dependent effects or 'floaters'. To cope with distractors, we advocate a form of robust estimation for NeRF training, modeling distractors in training data as outliers of an optimization problem. Our method successfully removes outliers from a scene and improves upon our baselines, on synthetic and real-world scenes. Our technique is simple to incorporate in modern NeRF frameworks, with few hyper-parameters. It does not assume a priori knowledge of the types of distractors, and is instead focused on the optimization problem rather than pre-processing or modeling transient objects. More results on our page https://robustnerf.github.io.

==> 3_method_OLD.tex <==
\section{Method}
\label{sec:method}
\vspace*{-0.1cm}

\AT{draft of method section structure}
\todo{\begin{itemize}
\item do nothing (L2): show failure
\item explain why.. view dependent effects can "cheat" 
\item use oracle segmenter... show perfect results
\item use L1 mipnerf: somewhat better (gives hope for robust?)
\item use robustness: slows down recon of high-freq (show and explain why); explain this is caused by an IID assumption of outliers (false, compare to oracle)
\item imitate the structure of the oracle {0,1} and smoothness works!
\end{itemize}}

We approach the problem of removing dynamic elements of a scene by treating them as outliers of an optimization. Since reconstructing the pixels attributed to this outliers will always have a greater loss compared to the consistent regions of an image, we advocate a robust optimization would be able to ignore the inconsistent pixels. Therefore, we can render a clean scene out of a series of images with moving objects without requiring extra modeling capacity. Also utilizing a robust optimizer rather than modeling the dynamic parts would increase the versatility of our method. When you aim for modeling the dynamic parts the number of dynamic parts are inherently limited by the capacity of your model. On the other hand, if you ignore the dynamic parts, there can be a completely different set of objects in each image and it would be no different for a robust optimizer.

We design a patch based robust optimizer that would keep the quality of the consistent parts of the scene while ignoring the pixels with large losses.
\TODO{formally describe the problem (non-fully static scene), re-iterate importance (no reliance on pre-trained models); employ \autoref{fig:ambiguity} to explain the problem and why it is difficult to model in a NeRF workload.}

To achieve our objective, we modify the NeRF technique in two critical ways:
\CIRCLE{1} we modify rendering equation by factoring the radiance term into a view-independent plus a collection of increasingly more powerful view-dependent effects, 
\CIRCLE{2} we carefully design learning losses to prevent mode collapse of this factorization.


\input{fig/architectures}


\subsection{Supervision}
As the model in \eq{nerfloss} has representation power strictly superior to that of a NeRF model, a natural question emerges: \textit{``how do we avoid mode collapse, where a single $\radiance_k$ explains the entire scene on its own?''}
The answer to this question is a careful design of the training losses, which we approach by building inspecting its extreme mode of operation: where a single \textit{static} scene with \textit{view-dependent} effects is encoded by a view-independent model. 


\input{fig/extreme1}
\paragraph{View-independent modeling of static scenes}
Consider a \textit{fully-static} scene and $K{=}0$, that is, where the only term in ??? is the \textit{view-independent} radiance.
If we use an L2 reconstruction loss to train the model as in \eq{nerfloss}, this results in view-dependent effects being modeled as so called 3D density ``floaters''; see \autoref{fig:extreme1}~(a).
This is due to the fact that L2 losses attempt to regress the mean appearance across all viewpoints, under the (generally faulty) assumption that appearance shifts are Gaussian-distributed.
To robustly regress an average view-dependence appearance, we can instead use a robust kernel~$\kernel_\kernelPar(.)$, where $\kernelPar$ is a parameter that controls the separation between inliers/outliers, and minimize the loss:
\begin{align}
\argmin_{\params} \:\:
\sum_{i} \expect_{\ray \sim \image_i}
\left[
\kernel_\kernelPar(\|\C_0(\ray; \params) - \C^\gt_i(\ray) \|_2) 
\right]  ,
\label{eq:medianappearance}
\end{align}
where a typical choice of kernel is Geman-McClure~\todo{[Geman]} or Welsh~\todo{[Welsh]}.
Employing the Welsh kernel, and setting $\kernelPar$ to aggressively filter outliers (e.g., \todo{$\kernelPar{=}.2$}), results in the outcomes illustrated in~\autoref{fig:extreme1}~(b).
\DF{mathematical form of estimator and alpha are not yet given.}

\DF{next sentence is unclear to me ... eg say something like: In addition to being useful for view-dependent effects, a robust estimator should also be effective in mitigating the adverse effects of moving objects  .... }
While our discussion assumed a fully-static scene, note how such an idea generalizes to non-static scenes as illustrated in~\autoref{fig:extreme1}~(c,d).


\paragraph{Losses}
Training our model \DF{Bump: Are we still talking about a model with K=0, or K>0?  Would it be useful to show L2 and robust estimater results here with K=0 right here in the paper for didactic reasons?} entails the minimization of two losses for \textit{each} of the $K$ layers in our architecture, the first for photometric consistency of the model with observed images, and the latter for behavior regularization:
\begin{align}
\argmin_{\params} \:\:
\sum_{i} \expect_{\ray \sim \image_i}
\left[ 
\sum_k \loss{rgb}(\params, k) 
+ 
\sum_k \loss{reg}(\params,k)
\right]
~.
\end{align}


\input{fig/kernels}
\paragraph{Designing the robust kernels}
The goal of a robust estimator is to down-weight or eliminate the influence of outliers on the estimated quantities of interest.
In our case, we specify the robust kernel $\Omega(\ray)$ in terms of a binary function that, ideally, only provides a non-zero derivative for rays that intersect consistent scene parts. 

Then we filter the model loss with our kernel $\Omega$ 
\begin{equation}
    \loss{rgb} = \sum_\ray \Omega(\ray)\, || \C(\ray; \params) - \C^\gt(\ray) || 
    ~.
\end{equation}
\DF related this to L1 robustness or the Welsh kernel.

We can also use $\Omega$ to set the constant value of the Geman-McLure or Welsh loss, e.g.,

\begin{equation}
    \alpha(\ray) = 0.8 \,  \Omega(\ray) + 1e-3 ~.
\end{equation}

We assume that if we train with only the rays that have the lower range of errors in a batch, the inconsistencies (i.e. outliers) will be filtered out.
Therefore, we filter the rays based on their reconstruction error. Let's define the sum of residual squares over the color channels as $\mathcal{S}$:
\begin{equation}
    \mathcal{S(\ray)} = \sum_i || \C_i(\ray; \params) - \C^\gt_i(\ray) ||^2
\end{equation}

The rays that point to dynamic objects have inconsistent predictions, yielding relatively large residuals within a batch. 
Lower bounding the rays too harshly will only prolong the training. Therefore, we set a threshold $\tau$ as the median of residual squares.
\DF{cite literature here.}
Only rays that have residual errors smaller than $\tau$ are considered to be inliers, and therefore have a non-zero loss gradient:
\begin{align}
    \tau &= \text{median}_\ray(S(\ray))\\
    \Omega(\ray) &= \mathcal{S}(\ray) < \tau
\end{align}

One drawback of this approach is that only using  a small fraction of rays in each batch will slow down training unnecessarily, depending on the distribution of outlier rays. 
To get a stronger learning signal we wish to improve the detection of outliers, thereby allowing us to increase the fraction of useful rays within a given batch.
To get a more reliable signal for outlier detection we incorporate context and neighbouring rays, exploiting the fact that outliers are not IID, but rather if one ray intersects a moving object, then it is more likely that neighbouring rays do as well, since most objects are spatially coherent.

To this end we identify the mislabeled consistent rays of the higher error range. 
We process image patches of $16\times16$ pixels together to design $\Omega(\ray)$. Spatial locality is an important factor in distinguishing dynamic parts of the scene versus view dependant artifacts such as shine and texture details.
First, we assume outlier objects does not occupy single rays alone. Therefore,
we smooth $\Omega$ to remove individual rays who are wrongly filtered by running a $3\times 3$ smoothing filter on $\Omega$. If more than $50\%$ of the $3\times 3$ patch around a ray have low residuals, then we select that ray as a consistent one.
\begin{align}
    \Omega_s &= \text{mean}_{3\times3} \Omega \\
    \Omega &= \Omega | (\Omega_s > 0.5)
\end{align}

Now we incorporate the context by looking at the $16\times16$ patch as a whole. If at least $60\%$ of the $16\times 16$ patch rays are inliers, then we consider the $8\times8$ patch in the center as a inlier set of rays.

\begin{align}
    \Omega_p &= \text{mean}_{16\times16} \Omega \\
    \Omega_c &= (\Omega_p > 0.6) \times \mathbb{J}_8 \\
    \Omega_c &= Pad_{16\times16}(\Omega_c, 0) \\
    \Omega &= \Omega | \Omega_c
\end{align}

\SSA{Done}

For our model to represent a super-set of the classical NeRF behavior, clearly not only the architecture but also the supervision loss ought to match.
Therefore, we expect the K-th layer to employ the classical L2 reconstruction loss:
\begin{align}
\loss{rgb}(\params, K) =
\kernel_{\kernelPar_K}(\|\C_K(\ray; \params) - \C^\gt_i(\ray) \|_2) 
\overset{?}{\approx}
\|\C_K(\ray; \params) - \C^\gt_i(\ray) \|_2^2 
\end{align}
leading to the question of  what robust kernel and choice of parameters satisfies $\kernel_{\kernelPar_K}(.) \approx (.)^2$.
As illustrated in \autoref{fig:kernels}~(left), we employ the Welsh kernel in our design:
\begin{equation}
    \kernel_\kernelPar(x) = 1 - e^{-.5 (x/c)^2} \, .
\end{equation}

We can then scale the square function to $f(x)=(1-e^{-.5}) \, x^2$ so that $f(1)\equiv \kernel_{\kernelPar{=}1}(1)$, and we recall that any monotonic mapping of an objective function does not change the locations of its minima.
As visualized in \autoref{fig:kernels}~(right), \textit{within} the $[0,1]$ range, the derivatives of the two functions will be, as desired, similar, leading to similarly trained NeRF models.

\newcommand{\footnoteOne}{\footnote{Consider a perfectly white static scene, with a non-static black object. In such a setting $\C_0(\ray)=1.0 \: \forall \ray$, hence to produce a black function along a ray, one of the layers $k{\geq1}$ needs to subtract radiance. Assuming, in the limit, the presence of a single layer, leads to the requirement $\C_0(\ray){\in}[-1,+1]$.}}
\paragraph{Regularizers and activation functions}
In the analysis we achieved the desired approximation in the $[0,1]$ range.
Classical NeRF models employ a sigmoid output activation to constrain $\C(\ray){\in}[0,1]$.
While we set $\C_0(\ray){\in}[0,1]$ via a similar activation, the subsequent terms cannot be purely additive\footnoteOne{}, hence we set $\C_0(\ray){\in}[-1,+1]$ via a $tanh(.)$ activation.
Given these activations our output ranges will be $\C_{0:k} \in [-k, k+1]$.
As this can lead to dead gradients (e.g. for $\kernelPar{=}1$ and $x{\gg}1$, as well as to a loss in L2 approximation behavior, we penalize the deviation of any of the outputs of the network from~$[0,1]$:
\begin{align}
\loss{reg}(\params, k) &= \barrier_{[0,1]}(\C_{0:k}(\ray; \params))
\label{eq:reg}
\end{align}
where $\barrier_{[a,b]}(x)$ is a quadratic barrier term penalizing its argument from exiting the range $[a,b]$, that is $\barrier_{[a,b]}(x){=}0 \:\: \forall x{\in}[a,b]$, $\barrier_{[a,b]}(x){=}(x-b)^2 \:\: \forall x{\geq}b$, and $\barrier_{[a,b]}(x){=}(x-a)^2 \:\: \forall x{\leq}a$.


\paragraph{Scheduling the robust kernel}
Another interesting aspect is understanding the effect of $\kernelPar$ on the inliers/outliers induced by a given kernel.
We can shed some understanding on this aspect by considering the inflection point of the kernel: the position along $[0,1]$ where we will transition from progressively increasing to progressively decreasing the gradients' magnitude:
\begin{equation}
\frac{\partial^2 \kernel_{\kernelPar}(x)}{\partial x^2} = \frac{(\kernelPar^2 - x^2)}{\kernelPar^4}\kernel_{\kernelPar}(x) = 0 \quad \text{s.t.} \quad x \in [0,1] \quad \rightarrow \quad x=c
\end{equation}
In other words, a \textit{linear} scheduling of $\kernelPar_k$ leads to a \textit{linear} distribution of inlier/outlier decision boundaries.
Experimentally, as we find that this scheduling does not distribute well the information across the $K$ representation heads, we employ a log-scale allocation:
\begin{align}
\loss{rgb}(\params, k) &= \kernel_{\kernelPar_k}(\|\C_k(\ray; \params) - \C^\gt_i(\ray) \|_2) 
\\
\kernelPar_k &= e^{k - K + 1}
\end{align}


\paragraph{Training modality}
One could train the architecture above sequentially, 
More specifically, by training $\C_0$ (to convergence), then training $\C_1$ (to convergence) while freezing $\C_0$, and iterate this scheme for other layers.
Instead, as illustrated in \autoref{fig:architectures}~(right), we opt for co-training all layers simultaneously via the injection of two \textit{stop-gradients}:
\begin{align}
\nabla_{\params} \left[ \C_{k}(\ray; \params) \right]
&\leftarrow
\nabla_{\params} \left[ \Sigma_{i=0}^K \C_{i}(\ray; \params) \right]
\quad &\forall k \in \left\{1,\cdots, K\right\}
\\
\nabla_{\params_k} \left[ \loss{rgb}(\params, k) \right]
&\leftarrow
\nabla_{\params} \left[ \loss{rgb}(\params, k) \right]
\quad &\forall k \in \left\{1,\cdots, K\right\}
\end{align}
where $\params_k$ refers to the training parameters of the k-th layer.
\TODO{and now motivate why we need \textit{both}, still a tad unclear to me, with words and perhaps an experiment?}







==> 4_results_OLD.tex <==
\clearpage
\section{Experiments}
\color{red}
\AT{have not edited this section}
\label{sec:experiments}
\vspace*{-0.1cm}

We experiment on both synthetic and real scenes, where in each image of the training at least one outlier object is present. The test ground truth images are always from unseen viewpoints without any outlier objects. For each scene we also gather a clean training dataset without any distractors to measure the upperbound of the achievable quality with our setup.

The real scene images are captured with a Canon DSLR camera and the camera intrinsics and extrinsics are inferred by running Colmap on all the images.
The Statue dataset has $255$ images. In each image a pink balloon is present at a random location. The images are taken from $360 ^{\circ}$ around the statue object in the middle. 
The statue-clean dataset has $161$ images around the statue object. In the statue-clean dataset the scene is completely static. 
\color{black}

\input{fig/psnr}
\input{fig/psnr2.tex}
\input{fig/ablation.tex}

\input{fig/trainimage}
\input{fig/resultsimage}
\input{fig/jitterimage.tex}
All the models are trained for 250,000 iterations.


\subsection{Comparison to transient radiance-fields}
Nerf-in-the-wild~\cite[Sec.~4.2]{nerfw} introduces \textit{transient} radiance-fields to model image-dependent radiance by conditioning training views on a (learnable, per image) latent code $\latent_i$.
This allows them to imbue the model with some capability to detect outliers, which they refer to as ``transient objects''.
This is achieved by modifying~\eq{nerfmodel} to obtain image-dependent density, radiance, and \textit{spatial uncertainty}~$\uncertainty(\position)$:
\begin{align}
\begin{rcases}
\radiance_i(\position, \dir) \!\!\!\!\!
&= \radiance(\position, \dir) + \radiance^\transient(\position, \dir; \latent_i)
\\
\density_i(\position)
&= \density(\position) + \density^\transient(\position; \latent_i)
\\
\uncertainty_i(\position)
&= \uncertainty_\text{min} + \uncertainty_i(\position; \latent_i)
\!\!
\end{rcases} 
\text{NeRFW}(\position, \dir ; \params, \latent_i)
\label{eq:nerfw}
\end{align}
where $\uncertainty_i(\position; \latent_i) \geq 0 $ (using a softplus activation layer), and $\uncertainty_\text{min}$ prevents division-by-zero, and where spatial uncertainty is rendered by using \textit{transient} densities \AT{why?}:
\begin{align}
\C_i(\ray; \params) = \render(\ray; \radiance_i(\cdot,\cdot), \density_i(\cdot))
\\
\uncertainty_i(\ray) = \render(\ray; \uncertainty_i(\cdot), \density^\transient(\cdot; \latent_i))
\end{align}
and then supervised i.i.d.\ per-ray, following the Bayesian framework in \cite{kendall2017uncertainties}, by the sum of three 
losses:
\begin{align}
\loss{nerfw}(\ray; \params, \{\latent_i\}) &= \sum_i
\mathcal{L}_\C^{\ray, i} +
\mathcal{L}_\uncertainty^{\ray, i} +
\mathcal{L}_\transient^{\ray, i}
\label{eq:nerfwloss}
\end{align}
The first two terms are the (shifted) negative log-likelihood of a distribution which assumes that scenes containing outliers are well modeled by a (per-pixel)~Gaussian distribution in image space:
\begin{align}
\mathcal{L}_\C^{\ray, i} &= \frac{1}{2 \uncertainty_i(\ray)^2} \cdot \| \C_i(\ray; \params) - \C_i(\ray) \|_2^2
\label{eq:loss-rgb-nerfw}
\\
\mathcal{L}_\uncertainty^{\ray, i} &= \log \uncertainty_i(\ray)
\vphantom{\frac{1}{2}}
\end{align}
and the term $\loss{reg}^\transient$ is a \textit{prior} that incentivizes the model to explain the data \textit{without} resorting to transient modeling:
\begin{align}
\mathcal{L}_\transient^{\ray, i} &= \lambda_\tau
\cdot
\expect_{\position \sim \ray} \left[ \density^\transient(\position; \latent_i) \right]
\end{align}
where $\lambda_\tau$ is a hyper-parameter controlling this trade-off.

\input{fig/histograms}
Generally speaking, assuming the residuals to be Gaussian does match reality (see~\autoref{fig:histograms}), resulting in a difficult-to-tune optimization process.
\DF{One could view the formulation sa a form of IRLS in which the form of the weight is determined by beta.  This downweights residuals when uncertainnty is high, e.g., as with a heavy tailed process. Of course it is a limited form of robust estimator perhaps, and doesn't capture spatial coherence of outliers, etc.  We should not claim it assumes Gaussian which doesn't match reality because in some sense so does IRLS.}
\AT{actually, it does capture spatial coherence, via the \textbf{uncertainty field}, which pushes in the inductive biases of MLPs?}

Recent extensions of this method, such as~\ddnerf~\cite{d2nerf}, combine static/transient model of density and radiance~\eq{nerfw}, with modern space-time models~\cite{hypernerf}, and priors that promote a separation of the environment into either empty space or solid surfaces~\cite{lolnerf}.
However, such models are limited to \textit{video} disentanglement; \todo{see Figure XX}.
\DF{rewrite paragraph more clearly.}


==> fig/architectures.tex <==
\begin{figure}[t]
\begin{center}
\includegraphics[width=\linewidth]{example-image-golden}
\end{center}
\caption{
\textbf{Architectures --}
(left) the classical NeRF architecture;
(right) our architecture.
\TODO{add the skip connection for view direction}
}
\label{fig:architectures}
\end{figure}


==> fig/extreme1.tex <==
\begin{figure}[t]
\begin{center}
\includegraphics[width=.49\linewidth]{example-image-golden}
\hfill
\includegraphics[width=.49\linewidth]{example-image-golden}
\\
\includegraphics[width=.49\linewidth]{example-image-golden}
\hfill
\includegraphics[width=.49\linewidth]{example-image-golden}
\end{center}
\caption{
\textbf{Extreme Setting \#1 --}
(a) \todo{L2 w/o view-depedent on static scene};
(b) \todo{robust w/o view-depedent on static scene};
(c) \todo{L2 w/o view-depedent on jitter scene};
(d) \todo{robust w/o view-depedent on jitter scene}.
}
\label{fig:extreme1}
\end{figure}


==> fig/jitterimage.tex <==
\begin{figure}
\centering
\includegraphics[width=\linewidth]{fig/jitter.jpeg}
\caption{Inference renderings from new viewpoints for L2, L1, and RobustNerf on the jitter dataset. During training three objects jitter at their place slightly while the other five are fixed. L1 model generates a cloud at the rough place of the jittering objects while \RobustNeRF successfully removes them. \AT{R2: why did you not include mipnerf?}}
\label{fig:jitter}
\end{figure}


==> fig/psnr.tex <==
\begin{table}[]
\resizebox{\linewidth}{!}{ %
\begin{tabular}{@{}lllllllll@{}}
\toprule
\multicolumn{1}{l|}{} & \multicolumn{4}{c|}{Statue} & \multicolumn{4}{c}{Android} \\ \midrule
\multicolumn{1}{l|}{Loss} & L2 & L1 & MipNerf360 & \multicolumn{1}{l|}{RobustNerf} & L2 & L1 & MipNerf360 & RobustNerf \\ \midrule
\multicolumn{1}{l|}{PSNR} & 19.09 & 19.55 & 19.64 & \multicolumn{1}{l|}{20.89} & 19.35 & 19.38 & 19.53 & 19.75 \\
\multicolumn{1}{l|}{SSIM} & 0.66 & 0.72 & 0.73 & \multicolumn{1}{l|}{0.75} & 0.65 & 0.66 & 0.66 & 0.67 \\
\multicolumn{1}{l|}{LPIPS} & 0.36 & 0.30 & 0.30 & \multicolumn{1}{l|}{0.28} & 0.40 & 0.40 & 0.40 & 0.38 \\ \midrule
\begin{tabular}[c]{@{}l@{}}PSNR\\ Clean\end{tabular} &  &  & 23.57 & 23.29 &  &  & 20.88 & 
\end{tabular}
} %
\caption{\textbf{PSNR} --
Quantitative results on the Statue and Android datasets. The oracle row shows the PSNR of the model trained on clean images without distractors as an upperbound.
\DF{Should we mention statistical efficiency with robustNERF given clean data?}
\AT{what do you mean?}
}
\label{tab:main}
\end{table}


==> fig/resultsimage.tex <==
\begin{figure}
\centering
\includegraphics[width=0.49\textwidth]{fig/results.jpeg}
\caption{\textbf{Qualitative results (novel view synthesis) --}.
When trained with L2, L1, MipNerf360, and RobustNerf.
\TODO{Add dataset names beside image}
\TODO{Add citations in caption}
\TODO{Transpose image? (vertical layout)}}
\label{fig:resultsimage}
\end{figure}

